Sources of capital growth

Data from national accounts show no effect of change in net saving or consumption, in ratio to market-value capital, on change in growth rate of market-value capital (capital acceleration). Thus it appears that capital growth and acceleration arrive without help from net saving or consumption restraint. We explore ways in which this is possible, and discuss implications for economic teaching and public policy

==> tables/tbl-reg_s.tex <==
\centering
\begin{tabularx}{\columnwidth}{lcc}
   \midrule 
   Regression of $s^*$ on \(g(K)\)             & 0.0771$^{***}$ &   \\   
   Regression of value shown on $\Delta g(K)$  &                & 0.0559$^{***}$\\   
                                               &                & (0.0057)\\   
    \\
   Observations                                & 1,826          & 1,574\\  
   R$^2$                                       & 0.84511        & 0.37071\\  
   Within R$^2$                                & 0.10669        & 0.27233\\  
    \\
   Year fixed effects                          & $\checkmark$   & $\checkmark$\\   
   Country fixed effects                       & $\checkmark$   & $\checkmark$\\   
   \bottomrule
\end{tabularx}
   \label{tbl-reg_s}


==> tables/tbl-wid_c_table.tex <==
\begin{table}[pos=h]
\caption{Regression of $- \Delta c^*$ and $\Delta q_c$ on $\Delta g(K)$ (Screen = 0.01). $H_0 \text{ per thrift theory: } \Delta g(K) \cong -\Delta c^* \& \Delta q_c \cong 0$}
\centering
\begin{tabularx}{\columnwidth}{lcc}
   \toprule
                                               & $-\Delta c^*$   & $\Delta q_c$ \\    
   \midrule 
   Regression of value shown on $\Delta g(K)$  & -0.3760$^{***}$ & 1.376$^{***}$\\   
                                               & (0.1055)        & (0.1055)\\   
    \\
   Observations                                & 1,548           & 1,548\\  
   R$^2$                                       & 0.53993         & 0.88294\\  
   Within R$^2$                                & 0.31853         & 0.86226\\  
    \\
   Year fixed effects                          & $\checkmark$    & $\checkmark$\\   
   Country fixed effects                       & $\checkmark$    & $\checkmark$\\   
   \bottomrule
\end{tabularx}
   \label{tbl-wid_c_table}
\end{table}
